Supporting Human Raters with the Detection of Harmful Content using Large Language Models

In this paper, we explore the feasibility of leveraging large language models (LLMs) to automate or otherwise assist human raters with identifying harmful content including hate speech, harassment, violent extremism, and election misinformation. Using a dataset of 50,000 comments, we demonstrate that LLMs can achieve 90% accuracy when compared to human verdicts. We explore how to best leverage these capabilities, proposing five design patterns that integrate LLMs with human rating, such as pre-filtering non-violative content, detecting potential errors in human rating, or surfacing critical context to support human rating. We outline how to support all of these design patterns using a single, optimized prompt. Beyond these synthetic experiments, we share how piloting our proposed techniques in a real-world review queue yielded a 41.5% improvement in optimizing available human rater capacity, and a 9--11% increase (absolute) in precision and recall for detecting violative content.

==> Makefile <==
all: main.pdf

main.pdf:  *.tex *.sty tables/*.tex figs/*.pdf *.bib
	pdflatex main
	bibtex main
	pdflatex main
	pdflatex main
	pdflatex main

clean:
	rm -f *.bak
	rm -f *~
	rm -f main.pdf
	rm -f main.ps
	rm -f *.log
	rm -f *.aux*
	rm -f *.dvi
	rm -f *.bbl
	rm -f *.blg
	rm -f *.idx
	rm -f *.out

rubber:
	rubber --pdf -Wall --warn misc main.tex
	rubber-info main.tex

watch:
	make rubber
	- while true; do \
	  	inotifywait -r -e DELETE_SELF -e MOVE_SELF -e MODIFY *.tex *.bib tables/*.tex figs/*; \
			make rubber; \
			sleep 1; \
		done

